Product Design Using Generative Adversarial Network: Incorporating Consumer Preference and External Data

The rise of generative artificial intelligence (AI) has facilitated automated product design but often neglects valuable consumer preference data within companies' internal datasets. Additionally, external sources such as social media and user-generated content (UGC) platforms contain substantial untapped information on product design and consumer preferences, yet remain underutilized. We propose a novel framework that transforms the product design paradigm to be data-driven, automated, and consumer-centric. Our method employs a semi-supervised deep generative architecture that systematically integrates multidimensional consumer preferences and heterogeneous external data. The framework is both generative and preference-aware, enabling companies to produce consumer-aligned designs with enhanced cost efficiency. Our framework trains a specialized predictor model to comprehend consumer preferences and utilizes predicted popularity metrics to guide a continuous conditional generative adversarial network (CcGAN). The trained CcGAN can directionally generate consumer-preferred designs, circumventing the expenditure associated with testing suboptimal candidates. Using external data, our framework offers particular advantages for start-ups or other resource-constrained companies confronting the ``cold-start" problem. We demonstrate the framework's efficacy through an empirical application with a self-operated photography chain, where our model successfully generated superior photo template designs. We also conduct web-based experiments to verify our method and confirm its effectiveness across varying design contexts.

==> adoption_number.tex <==
\scalebox{0.9}{
	\begin{tabular}{lcccc} \hline \hline 
		                      & Mean     & Median   & Min   & Max              \\ \hline 
		& \multicolumn{4}{c}{Chinese-traditional Theme}  \\ \cline{2-5}
		DCGAN                 & 705.475   & 776.0  & 12      &  929                 \\ 
		cDCGAN (class=4)      & 765.07    & 820.0  & 143     & 923                  \\
        \hline
		& \multicolumn{4}{c}{Graffiti Theme} \\ \cline{2-5}
		DCGAN                 & 763.66   & 809.0  &  115  & 907    \\
		cDCGAN (class=4)      & 770.845  & 813.5  &  65   & 917    \\
		\hline \hline 
	\end{tabular}
}

==> class_label.tex <==
%\begin{tabular}{lcccc}
%\toprule
%\textbf{Theme} & \textbf{Class Label}=1 & \textbf{Class Label}=2 & %\textbf{Class Label}=3 & \textbf{Class Label}=4 \\
%\midrule
%Graffiti  &  & 0.808 & 0.184 & 0.201 \\
%\bottomrule
%\end{tabular}


\begin{tabular}{lcc}
\toprule
\textbf{Theme} & \textbf{Graffiti}           & \textbf{Chinese Traditional} \\
\midrule
Class label=1  & \# of adoption $\in [6, 711]$   & \# of adoption $\in [22, 719]$  \\
Class label=2  & \# of adoption $\in (712, 802]$ & \# of adoption $\in (719, 827]$  \\
Class label=3  & \# of adoption $\in (802, 858]$ & \# of adoption $\in (827, 874.5]$  \\
Class label=4  & \# of adoption $\in (858, 923]$ & \# of adoption $\in (874.5, 925]$  \\
\bottomrule
\end{tabular}


==> prediction_acc.tex <==
%\scalebox{0.9}{
%\begin{tabular}{lcccc} \hline \hline 
%    \textbf{Choice Prediction Task} & \textbf{Acc.} & \textbf{Balanced Acc.} & \textbf{FNR} & \textbf{FPR} \\ %\hline 
%    Random Forest (Under-Sampling)  & 0.801 & 0.808 & 0.184 & 0.201 \\
%    \hline \hline 
%    \footnotetext{This table presents the accuracy rate, balanced accuracy rate, false negative rate, and false positive rate for the consumer choice model prediction result on the test set.}
%\end{tabular}
%}


\begin{tabular}{lcccc}
\hline\hline
\textbf{Choice Prediction Task} & \textbf{Acc.} & \textbf{Balanced Acc.} & \textbf{FNR} & \textbf{FPR} \\
\hline
Random Forest (Up-Sampling)  & 0.793 & 0.791 & 0.212 & 0.206 \\
\hline \hline
\end{tabular}


==> prediction_acc2.tex <==
%\scalebox{0.9}{
%\begin{tabular}{lcccc} \hline \hline 
%    \textbf{Choice Prediction Task} & \textbf{Acc.} & \textbf{Balanced Acc.} & \textbf{FNR} & \textbf{FPR} \\ %\hline 
%    Random Forest (Under-Sampling)  & 0.801 & 0.808 & 0.184 & 0.201 \\
%    \hline \hline 
%    \footnotetext{This table presents the accuracy rate, balanced accuracy rate, false negative rate, and false positive rate for the consumer choice model prediction result on the test set.}
%\end{tabular}
%}


\begin{tabular}{lcccc}
\hline
\textbf{Prediction Model} & \textbf{Acc.} & \textbf{Balanced Acc.} & \textbf{FNR} & \textbf{FPR} \\
\hline
1 (Internal preference only)          & 0.793 & 0.791 & 0.212 & 0.206 \\
2 (Internal and external preferences) & 0.806 & 0.825 & 0.148 & 0.202 \\

\hline
\end{tabular}


==> sorting_patterns.tex <==
\begin{table}[H]
\caption{\textbf{Sorting Patterns of Coder Characteristics on Project Characteristics}}
\centering
\begin{threeparttable}
\label{tab:my-table}
{\footnotesize
\begin{tabular}{lccccc}
\hline
\hline
                                                         & (1)                                                            & (2)                                                           & (3)                                                             & (4)                                                                   & (5)      \\
                                                         & \begin{tabular}[c]{@{}c@{}}Total  Cash\\  Rewards\end{tabular} & \begin{tabular}[c]{@{}c@{}}Daily  Cash\\  Reward\end{tabular} & \begin{tabular}[c]{@{}c@{}}No. of \\ Registrations\end{tabular} & \begin{tabular}[c]{@{}c@{}}DR  Points \\ (after 05/2006)\end{tabular} & Duration \\\hline
                                                         &                                                                &                                                               &                                                                 &                                                                       &          \\
Rating Score                                             & -0.02***                                                       & -0.00***                                                      & 0.00                                                            & 0.01*                                                                 & -0.00    \\
                                                         & (0.01)                                                         & (0.00)                                                        & (0.00)                                                          & (0.00)                                                                & (0.00)   \\
Experience                                               & 0.91***                                                        & 0.23***                                                       & -0.09***                                                        & 0.22***                                                               & -0.00    \\
                                                         & (0.13)                                                         & (0.03)                                                        & (0.01)                                                          & (0.08)                                                                & (0.00)   \\
China                                                    & -17.77***                                                      & -2.85**                                                       & 0.34                                                            & -4.05                                                                 & -0.04    \\
                                                         & (5.42)                                                         & (1.23)                                                        & (0.31)                                                          & (3.62)                                                                & (0.04)   \\
Canada/US                                                & 0.81                                                           & -1.78                                                         & 1.08*                                                           & 9.08*                                                                 & -0.02    \\
                                                         & (9.84)                                                         & (1.53)                                                        & (0.59)                                                          & (5.16)                                                                & (0.06)   \\
India                                                    & 9.09                                                           & -0.90                                                         & 0.15                                                            & 7.33                                                                  & 0.04     \\
                                                         & (11.58)                                                        & (1.89)                                                        & (0.71)                                                          & (7.60)                                                                & (0.08)   \\
Constant                                                 & 122.62***                                                      & 14.62***                                                      & 18.27***                                                        & -16.01**                                                              & 13.02*** \\
                                                         & (10.02)                                                        & (1.86)                                                        & (1.43)                                                          & (6.71)                                                                & (0.13)   \\
\begin{tabular}[c]{@{}l@{}}Year-Month \\ FE\end{tabular} & Y                                                              & Y                                                             & Y                                                               & Y                                                                     & Y        \\
                                                         &                                                                &                                                               &                                                                 &                                                                       &          \\\hline
Observations                                             & 9,778                                                          & 9,757                                                         & 10,052                                                          & 10,052                                                                & 10,049   \\
R-squared                                                & 0.28                                                           & 0.22                                                          & 0.25                                                            & 0.69                                                                  & 0.43 \\   
\hline
\hline
\end{tabular}}
\begin{tablenotes}
\scriptsize
\item Notes: Robust standard errors in parentheses;  * p $<$ 0.05, ** p$<$0.01, *** p$<$0.001.             
\end{tablenotes}
\end{threeparttable}
\end{table}

==> sum_stat_consumer.tex <==
\begin{tabular}{lccccc} \hline \hline 
    Variable & Mean & Std. Dev. & Min & Max & Obs \\ \hline 
    \# of photos taken & 9.25 & 8.70 & 1 & 104 & 2195 \\
    \# of photos printed & 3.50 & 5.16 & 0 & 48 & 2195 \\
    \# of themes selected & 3.57 & 2.94 & 1 & 34 & 2195 \\
    \# of templates selected & 7.67 & 7.17 & 1 & 81 & 2195\\
    Amount of money spent (CNY) & 36.08 & 23.53 & 0 & 209.7 & 2195 \\
    Amount of time spent (min) & 20.28 & 19.26 & 0 & 180 & 2195 \\
    \hline \hline 
\end{tabular}


==> theme_adopt.tex <==
\begin{tabular}{lcc} \hline \hline 
	Most popular themes    & Adoption times\\
	\hline
	Chinese traditional    & 900\\
	Pretend to be in Japan & 875\\
	Instagram style        & 776\\
	Good times (cozy home) & 666\\
	Cartoon style          & 665\\
	Cherry blossom seasons & 610\\
	Plum blossom           & 377\\
	Graffiti               & 295 \\
	Graffiti II            & 222\\
	\hline \hline
\end{tabular}
